Memory Efficient GPU-based Label Propagation Algorithm (LPA) for Community Detection on Large Graphs

Community detection involves grouping nodes in a graph with dense connections within groups, than between them. We previously proposed efficient multicore (GVE-LPA) and GPU-based ($\nu$-LPA) implementations of Label Propagation Algorithm (LPA) for community detection. However, these methods incur high memory overhead due to their per-thread/per-vertex hashtables. This makes it challenging to process large graphs on shared memory systems. In this report, we introduce memory-efficient GPU-based LPA implementations, using weighted Boyer-Moore (BM) and Misra-Gries (MG) sketches. Our new implementation, $\nu$MG8-LPA, using an 8-slot MG sketch, reduces memory usage by 98x and 44x compared to GVE-LPA and $\nu$-LPA, respectively. It is also 2.4x faster than GVE-LPA and only 1.1x slower than $\nu$-LPA, with minimal quality loss (4.7%/2.9% drop compared to GVE-LPA/$\nu$-LPA).

==> src/fig-optpickstepbm.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure{
    \label{fig:optpickstepbm--runtime}
    \includegraphics[width=0.98\linewidth]{out/optpickstepbm-runtime.pdf}
  }
  \subfigure{
    \label{fig:optpickstepbm--modularity}
    \includegraphics[width=0.98\linewidth]{out/optpickstepbm-modularity.pdf}
  } \\[-2ex]
  \caption{Relative Runtime and Modularity of obtained communities on varying \textit{Pick-Less (PL)} step from $1$ to $8$ for $\nu$BM-LPA, i.e., allowing the community label of each vertex to change only if the selected label is smaller than the current label, in every iteration (when $PL=1$), or once every $8$ iterations (when $PL=8$) --- starting from the first iteration.}
  \label{fig:optpickstepbm}
\end{figure}


==> src/fig-optpickstepmg.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure{
    \label{fig:optpickstepmg--runtime}
    \includegraphics[width=0.98\linewidth]{out/optpickstepmg-runtime.pdf}
  }
  \subfigure{
    \label{fig:optpickstepmg--modularity}
    \includegraphics[width=0.98\linewidth]{out/optpickstepmg-modularity.pdf}
  } \\[-2ex]
  \caption{Relative Runtime and Modularity of obtained communities on varying \textit{Pick-Less (PL)} step from $1$ to $8$ for $\nu$MG8-LPA, i.e., allowing the community label of each vertex to change only if the selected label is smaller than the current label, in every iteration (when $PL=1$), or once every $8$ iterations (when $PL=8$) --- starting from the first iteration.}
  \label{fig:optpickstepmg}
\end{figure}

